Blend: A Unified Data Discovery System

Most research on data discovery has so far focused on improving individual discovery operators such as join, correlation, or union discovery. However, in practice, a combination of these techniques and their corresponding indexes may be necessary to support arbitrary discovery tasks. We propose BLEND, a comprehensive data discovery system that supports existing operators and enables their flexible pipelining. BLEND is based on a set of lower-level operators that serve as fundamental building blocks for more complex and sophisticated user tasks. To reduce the execution runtime of discovery pipelines, we propose a unified index structure and a rule-based optimizer that rewrites SQL statements into low-level operators when possible. We show the superior flexibility and efficiency of our system compared to ad-hoc discovery pipelines and stand-alone solutions.

==> charts_and_tables/code_kw.tex <==
\begin{lstlisting}[language=SQL, caption={SQL implementation of the keyword seeker.}, label={sql:kw}, escapechar=|]
SELECT TableId FROM AllTables |\label{codeline_kw_select}|
WHERE CellValue IN (Q) |\label{codeline_kw_where}|
GROUP BY TableId |\label{codeline_kw_group}|
ORDER BY COUNT(DISTINCT CellValue) DESC |\label{codeline_kw_order}|
LIMIT K;    |\label{codeline_kw_limit}|
\end{lstlisting} 

==> charts_and_tables/code_overlap.tex <==
% \begin{figure}[H]
% \centering
% {\footnotesize
% \begin{BVerbatim}[commandchars=\\\{\}] 
% \textcolor{purple}{SELECT} TableId \textcolor{purple}{FROM} AllTables
% \textcolor{purple}{WHERE} CellValue \textcolor{orange}{IN} (Q) 
% \textcolor{purple}{GROUP BY} TableId
% \textcolor{purple}{ORDER BY} \textcolor{blue}{COUNT}(DISTINCT CellValue) \textcolor{purple}{DESC} 
% \textcolor{purple}{LIMIT} K;
% \end{BVerbatim}
% }
% \caption{SQL implementation of the value overlap seeker.}
% \label{sql:overlap}
% \end{figure}

\begin{lstlisting}[language=SQL, caption={SQL implementation of the value overlap seeker.}, label={sql:overlap}, escapechar=|]
SELECT TableId FROM AllTables |\label{codeline_overlap_select}|
WHERE CellValue IN (Q) |\label{codeline_overlap_where}|
GROUP BY TableId |\label{codeline_overlap_group}|
ORDER BY COUNT(DISTINCT CellValue) DESC |\label{codeline_overlap_order}|
LIMIT K;    |\label{codeline_overlap_limit}|
\end{lstlisting} 

==> charts_and_tables/code_rewriting.tex <==
\begin{lstlisting}[language=SQL, caption={Appending the MC query with a limiting predicate.}, label={sql:rewriting}, escapechar=|]
WHERE Q1_index_hits.TableId IN (|$IR_{SC}$|) |\label{codeline_rewriting}|
\end{lstlisting} 

==> charts_and_tables/code_union.tex <==
% \begin{figure}
% \centering
% {\footnotesize
% \begin{BVerbatim}[commandchars=\\\{\}]  
% \textcolor{gray}{1} \textcolor{purple}{def} \textcolor{blue}{UnionPlan}(dataset, k=\textcolor{orange}{10}) 
% \textcolor{gray}{2}     plan = \textcolor{red}{PlanClass}()
% \textcolor{gray}{3}     input_element = \textcolor{red}{Input}(dataset)
% \textcolor{gray}{4}     plan.\textcolor{red}{add}(\textcolor{olive}{'input'}, input_element)
% \textcolor{gray}{5}     \textcolor{purple}{for} clm_name \textcolor{purple}{in} dataset.columns:
% \textcolor{gray}{6}         element = Seekers.Seekers.\textcolor{red}{Overlap}(dataset[clm_name], k)
% \textcolor{gray}{7}         plan.\textcolor{red}{add}(clm_name, element, [\textcolor{olive}{'input'}])
% \textcolor{gray}{8}     plan.\textcolor{red}{add}(\textcolor{olive}{'counter'}, Combiners.\textcolor{red}{Counter}(), dataset.columns, k)
% \textcolor{gray}{9}     plan.\textcolor{red}{add}(\textcolor{olive}{'terminal'}, \textcolor{red}{Terminal}(), [\textcolor{olive}{'counter'}])
% \end{BVerbatim}
% }
% \caption{\system User API for the union discovery plan.}
% \label{code:union}
% \end{figure}


\begin{lstlisting}[language=Python, caption={\system User API for the union discovery plan.}, label={code:union}, escapechar=|]
def UnionPlan(dataset, K=10) 
    plan = Plan()|\label{codeline_union_plan}|
    input_element = Input(dataset)|\label{codeline_union_input}|
    plan.add('input', input_element)|\label{codeline_union_add_input}|
    for clm_name in dataset.columns:|\label{codeline_union_for}|
        element = Seekers.SC(dataset[clm_name], K|$'$|)
        plan.add(clm_name, element, ['input'])|\label{codeline_union_addoverlap}|
    plan.add('counter', Combiners.Counter(K), dataset.columns)|\label{codeline_union_add_combiner}|
    plan.add('terminal', Terminal(), ['counter'])|\label{codeline_union_add_terminal}|
\end{lstlisting}

==> charts_and_tables/new_experiments/components.tex <==
\begin{table}[]
     \footnotesize
    \centering
    \caption{Bottleneck analysis between \system and Baselines. The baseline for Single join is  Josie~\cite{DBLP:conf/sigmod/ZhuDNM19}, for MC Join is MATE~\cite{DBLP:journals/pvldb/EsmailoghliQA22}, for Union is Starmie~\cite{DBLP:journals/pvldb/FanWLZM23}, for correlation is QCR~\cite{DBLP:conf/icde/SantosBMF22}, and for augmentation is DataXFormer~\cite{abedjan2015dataxformer}.}
    % \vspace{-.2cm}
    \label{tab:components}
\begin{tabular}{r|rrr|rrr}
%\toprule

\textit{\textbf{Task}} & \multicolumn{3}{c|}{\textit{\textbf{{\system}}}}&  \multicolumn{3}{c}{\textit{\textbf{{Baseline}}}}
 \\

&\multicolumn{1}{c}{\textbf{DB}}&\multicolumn{1}{c}{\textbf{Load}}&\multicolumn{1}{c|}{\textbf{Mem}}&\multicolumn{1}{c}{\textbf{DB}}&\multicolumn{1}{c}{\textbf{Load}}&\multicolumn{1}{c}{\textbf{Mem}}\\
\toprule
Single Join  & 99.3\% & 0.0\% & 0.7\% & 47.0\%& 21.7\% & 31.3\%\\
MC Join  & 23.7\% & 14.3\% & 62.0\% & 12.6\%& 68.2\% & 19.2\%\\
Union  & 94.5\% & 0.0\% & 5.5\% & - & 2.7\% & 97.3\%\\
Correlation  & 100.0\% & 0.0\% & 0.0\% & 47.1\% & 0.0\% & 53.9\%\\
Augmentation  & 100.0\% & 0.0\% & 0.0\% & 99.7\% & 0.3\% & 0.0\%\\
\toprule
\end{tabular}
\end{table}

==> charts_and_tables/new_experiments/correlation_runtime.tex <==
\begin{table}
\caption{Runtime comparison between \system and QCR-based baseline~\cite{DBLP:conf/icde/SantosBMF22}}
\centering
\begin{tabular}{cccc}
\hline
\textbf{Correlation} & \textbf{Full Time} & \textbf{Execution Time} & \textbf{Fetch Time} \\
\hline
Baseline & 0.933970 & 0.324388 & 0.000196 \\
\system & 42.504417 & 42.502854 & 0.000138 \\
\hline
\end{tabular}
\label{tab:correlation_runtimes}
\end{table}

==> charts_and_tables/new_experiments/optimizer_runtime.tex <==
\begin{table}
\footnotesize
\caption{Efficiency evaluation of the plan optimizer.}
\centering
\begin{tabular}{l||r|r}
\textbf{Task} & \textbf{\thead{\system \\ with optimizer}} & \textbf{\thead{\system \\ without optimizer}} \\
\toprule
\textbf{Multi-Objective}&5.5&5.5\\
\textbf{Data Imputation}&\textbf{0.19}&0.26\\
\textbf{Feature Discovery}&\textbf{9.0}&16.3\\
\textbf{With Negative Examples}&\textbf{14.2}&111.9\\

% Synthetic & 45\% & 45\% & 69\% & 69\% \\
\hline
\end{tabular}
\label{tab:optimizer}
\end{table}

==> charts_and_tables/new_experiments/union_precision_larger_k.tex <==
\begin{table*}[]
     \footnotesize
    \centering
    \caption{Quality comparison between \system and STARMIE for .}
    % \vspace{-.2cm}
    \label{tab:union_quality_large_k}
\begin{tabular}{r|rrr|rrr||rrr|rrr}
%\toprule

 & \multicolumn{6}{c||}{\textit{\textbf{{K=50}}}}& \multicolumn{6}{c}{\textit{\textbf{{K=100}}}}
 \\

\textit{\textbf{Lake}} & \multicolumn{3}{c|}{\textit{\textbf{{\system}}}}&  \multicolumn{3}{c||}{\textit{\textbf{{STARMIE}}}}& \multicolumn{3}{c|}{\textit{\textbf{{\system}}}}&  \multicolumn{3}{c}{\textit{\textbf{{STARMIE}}}}
 \\

&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{R@K}}&\multicolumn{1}{c|}{\textbf{MAP}}&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{R@K}}&\multicolumn{1}{c||}{\textbf{MAP}}
&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{R@K}}&\multicolumn{1}{c|}{\textbf{MAP}}&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{R@K}}&\multicolumn{1}{c}{\textbf{MAP}}\\
\toprule
TUS  & \textbf{96\%} & \textbf{23\%} & \textbf{95\%} & 37\% & 09\% & 63\% & \textbf{96\%} & \textbf{44\%} & \textbf{96\%} & 24\% & 12\% & 47\%\\
TUS Large & \textbf{83\%} & \textbf{15\%} & \textbf{84\%} & 45\% & 08\% & 72\% & \textbf{85\%} & \textbf{29\%} & \textbf{85\%} & 27\% & 09\% & 53\%\\
\toprule
\end{tabular}
\end{table*}

==> charts_and_tables/new_experiments/union_precision_starmie_paper.tex <==
\begin{table*}[]
     \footnotesize
    \centering
    \caption{Quality comparison between \system and STARMIE.}
    % \vspace{-.2cm}
    \label{tab:union_quality}
\begin{tabular}{r|rrr|rrr||rrr|rrr}
%\toprule

 & \multicolumn{6}{c||}{\textit{\textbf{{K=10}}}}& \multicolumn{6}{c}{\textit{\textbf{{K=20}}}}
 \\

\textit{\textbf{Lake}} & \multicolumn{3}{c|}{\textit{\textbf{{\system}}}}&  \multicolumn{3}{c||}{\textit{\textbf{{STARMIE}}}}& \multicolumn{3}{c|}{\textit{\textbf{{\system}}}}&  \multicolumn{3}{c}{\textit{\textbf{{STARMIE}}}}
 \\

&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{Recall}}&\multicolumn{1}{c|}{\textbf{MAP}}&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{Recall}}&\multicolumn{1}{c||}{\textbf{MAP}}
&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{Recall}}&\multicolumn{1}{c|}{\textbf{MAP}}&\multicolumn{1}{c}{\textbf{P@K}}&\multicolumn{1}{c}{\textbf{Recall}}&\multicolumn{1}{c}{\textbf{MAP}}\\
\toprule
SANTOS  & 92\% &  70\% &  94\% &  \textbf{98\%} &  \textbf{74\%} &  \textbf{99\%} &  100\% &  89\% &  94\% &  \% &  \% &  \%\\
TUS  & 94\% &  \textbf{05\%} &  94\% &  \textbf{99\%} &  04\% &  \% &  95\% &  \textbf{10\%} &  94\% &  \textbf{98\% }&  09\% &  \%\\
TUS Large & 94\% &  04\% &  94\% &  \textbf{100\%} &  04\% &  \% &  94\% &  07\% &  94\% &  \textbf{99\%} &  \textbf{08\%} &  \% \\
\toprule
 & \multicolumn{6}{c||}{\textit{\textbf{{K=50}}}}& \multicolumn{6}{c}{\textit{\textbf{{K=100}}}}
 \\
TUS  & 96\% & \textbf{24\%} & 95\% & \textbf{98\%} & 23\% & \% & 93\% & 43\% & 92\% & \% & \% & \%\\
TUS Large & 92\% & 17\% & 93\% & 92\% & \textbf{21\%} & \% & 92\% & 32\% & 92\% & \% & \% & \%\\
 
\toprule
\end{tabular}
\end{table*}

==> charts_and_tables/temp_code.tex <==

\begin{lstlisting}[language=Python, caption={Building search plan in \system.}, label={code:augmentation_by_example}, escapechar=|]
def DiscoveryPlan(df, K):
    plan = Plan()
    inputs = Input([df]) 
    plan.add('input', inputs) 
    # Join Search Title
    title_seeker = Seekers.SC(inputs.elements[0].movie_title, K)
    plan.add('title', title_seeker, ['input']) 
    # Join Search Director Name
    director_seeker = Seekers.SC(inputs.elements[0].director, K)
    plan.add('director', director_seeker, ['input']) 
    # Feature Engineering
    feature_seeker = Seekers.Correlation(inputs.elements[0].movie_title, inputs.elements[0].director, K) 
    plan.add('feature', feature_seeker, ['input']) 
    plan.add('intersection', Combiners.Intersection(K), ['title', 'director', 'feature']) 
    plan.add('terminal', Terminal(), ['intersection']) 
dataframe = pd.read_csv('data/movie.csv')
plan = DiscoveryPlan(dataframe, 10)
plan.run()
\end{lstlisting}

==> charts_and_tables/temp_code_2.tex <==
\begin{lstlisting}[language=Python, caption={Building search plan in \system.}, label={code:augmentation_by_example}, escapechar=|]
def DiscoveryPlan(included_kws, excluded_kws, K):
    plan = Plan()
    inputs = Input([included_kws, excluded_kws]) 
    plan.add('input', inputs) 
    # Included tables
    inclusion_seeker = Seekers.SC(inputs.elements[0], K)
    plan.add('included', inclusion_seeker, ['input']) 
    # Excluded tables
    exclusion_seeker = Seekers.SC(inputs.elements[1], K)
    plan.add('excluded', exclusion_seeker, ['input']) 
    plan.add('difference', Combiners.Difference(K), ['included', 'excluded']) 
    plan.add('terminal', Terminal(), ['difference']) 
included_kws = ['Bayern Munich', 'Eintracht Frankfurt', 'FC Koln', 'Hertha Berlin']
excluded_kws = ['Barcelona', 'Paris Saint Germain', 'Arsenal', 'Juventus']
plan = DiscoveryPlan(included_kws, excluded_kws, 10)
plan.run()
\end{lstlisting}

==> charts_and_tables/temp_code_alternate_2.tex <==

\begin{lstlisting}[language=Python, caption={Building search plan in \system.}, label={code:augmentation_by_example}, escapechar=|]
def DataDiscovery(included_keywords, excluded_keywords, K=10):
    connection = vertica_python.connect(
        host=config['Database']['host'],
        port=config['Database']['port'],
        user=config['Database']['user'],
        password=config['Database']['password'],
        database=config['Database']['dbname'],
        session_label='some_label',
        read_timeout=60000,
        unicode_error='strict',
        ssl=False,
        use_prepared_statements=False)

    cur = connection.cursor()

    # Included tables
        cur.execute('SELECT TableId FROM All_Tables '
                'WHERE CellValue IN \'{}\' '
                'GROUP BY TableId '
                'ORDER BY '
                'COUNT(DISTINCT CellValue) DESC;'
                .format(', '.join(included_keywords)))
    included_table_query = [row[0] for row in cur.fetchall()]

    # Excluded tables
    cur.execute('SELECT TableId FROM All_Tables '
                'WHERE CellValue IN \'{}\' '
                'GROUP BY TableId '
                'ORDER BY '
                'COUNT(DISTINCT CellValue) DESC;'
                .format(', '.join(excluded_keywords)))
    excluded_table_query = [row[0] for row in cur.fetchall()]

    desired_tables = [table for table in included_table_query if table not in excluded_table_query]
    return desired_tables[:K]

included_kw = ['Bayern Munich', 'Eintracht Frankfurt', 'FC Koln', 'Hertha Berlin']
excluded_kw = ['Barcelona', 'Paris Saint Germain', 'Arsenal', 'Juventus']
tables = DataDiscovery(included_kw, excluded_kw, 10)
\end{lstlisting}

==> charts_and_tables/temp_code_alternative.tex <==

\begin{lstlisting}[language=Python, caption={Building search plan in \system.}, label={code:augmentation_by_example}, escapechar=|]
def DataDiscovery(df ,K=10):
    connection = vertica_python.connect(
        host=config['Database']['host'],
        port=config['Database']['port'],
        user=config['Database']['user'],
        password=config['Database']['password'],
        database=config['Database']['dbname'],
        session_label='some_label',
        read_timeout=60000,
        unicode_error='strict',
        ssl=False,
        use_prepared_statements=False)

    cur = connection.cursor()

    # Join Search Title
    movie_titles = list(df['movie_title'])
    cur.execute('SELECT TableId FROM All_Tables '
                'WHERE CellValue IN \'{}\' '
                'GROUP BY TableId '
                'ORDER BY COUNT(DISTINCT CellValue) DESC;'.format(', '.join(movie_titles)))
    list_of_joinable_table_ids_to_titles = [row[0] for row in cur.fetchall()]

    # Join Search Director Name
    director_names = list(df['director_names'])
    cur.execute('SELECT TableId FROM All_Tables '
                'WHERE CellValue IN \'{}\' '
                'GROUP BY TableId '
                'ORDER BY COUNT(DISTINCT CellValue) DESC;'.format(', '.join(director_names)))
    list_of_joinable_table_ids_directors = [row[0] for row in cur.fetchall()]

    correlating_columns = {}
    # Feature Engineering
    for table_id in list_of_joinable_table_ids_to_titles:
        fetch_table_query = 
                    'SELECT CellValue, ' \
                    'ColumnId, RowId ' \
                    'FROM All_Tables ' \
                    'WHERE TableId = {}'.format(table_id)
        table_content = cur.fetchall(fetch_table_query)
        candidate_table_df = pd.DataFrame(table_content, columns=['CellValue', 'ColumnId', 'RowId'])
        candidate_table_df = candidate_table_df.pivot(index='RowId', columns='ColumnId', values='CellValue')
        candidate_table_df.index.name = None
        candidate_table_df.columns.name = None
        joinable_column_query = 'SELECT ColumnId ' \
                          'FROM All_Tables ' \
                          'WHERE TableId = {} ' \
                          'AND CellValue IN {} ' \
                          'GROUP BY ColumnId ' \
                          'ORDER BY COUNT(DISTINCT ' \
                          'CellValue) DESC;'
                          .format(table_id, ','.join(movie_titles))
        joinable_column = [row[0] for row in cur.fetchall(joinable_column_query)][0]
        merged_dfs = df.merge(candidate_table_df, how='inner', left_on='movie_title', right_on=joinable_column)
        correlation_results = merged_dfs.corr(method='pearson').abs()
        top_correlating_columns = correlation_results.loc['imdb_score'].sort_values(ascending=False)
        top_correlating_column = top_correlating_columns.index[0]
        correlating_columns[table_id] = top_correlating_columns[0]
    correlating_tables = {k: v for k, v in sorted(correlating_columns.items(), key=lambda item: item[1], reverse=True)[:K]}
    return set(list_of_joinable_table_ids_to_titles)\
        .intersection(set(list_of_joinable_table_ids_directors))\
        .intersection(set(correlating_tables))

dataframe = pd.read_csv('data/movie.csv')
tables = DataDiscovery(dataframe, 10)
\end{lstlisting}

==> charts_and_tables/temp_code_sql_2.tex <==

\begin{lstlisting}[language=SQL, caption={Building search plan in \system.}, label={code:augmentation_by_example}, escapechar=|]
SELECT TableId 
FROM All_Tables 
WHERE CellValue IN ('Bayern Munich', 'Eintracht Frankfurt', 'FC Koln', 'Hertha Berlin') 
AND 
    TableId NOT IN (
        SELECT TableId 
        FROM All_Tables 
        WHERE CellValue IN ('Barcelona', 'Paris Saint Germain', 'Arsenal', 'Juventus')
        GROUP BY TableId 
        ORDER BY COUNT(DISTINCT CellValue) DESC;
    ) 
GROUP BY TableId 
ORDER BY COUNT(DISTINCT CellValue) DESC;
\end{lstlisting}
